Historian: Reducing Manual Validation in APR Benchmarking via Evidence-Based Assessment

Assessing the correctness of patches generated by Automated Program Repair (APR) is a major bottleneck. Manual validation is labor-intensive and limited: exact matching overlooks valid variants, while semantic inspection is subjective and hard to reproduce. Existing Automated Patch Correctness Assessment (APCA) often relies on opaque predictive models that treat each patch as novel, repeatedly re-assessing semantically redundant patches. Our analysis of a large corpus of tool-generated patches reveals a duality: about 39% of unique correct patches are syntactic clones, suggesting opportunities for automation, yet about 65% of bugs have multiple distinct correct fixes, making single-reference assessment insufficient. We present Historian, a framework that leverages Large Language Models to perform multi-reference comparisons against a knowledge base of historically validated patches, producing traceable, evidence-based verdicts while conservatively isolating novel cases as Unknown. In leave-one-tool-out evaluation, Historian achieves 95.0% coverage with 88.4% accuracy, reducing manual validation to 5% of patches. As an evidence-based pre-filter, enhancing the accuracy of standalone APCA tools by up to 21.8% and enabling a hybrid pipeline with 86.2% overall accuracy and 100% coverage. A longitudinal analysis of tool-generated patches (2020-2024) shows that redundancy in repair attempts is common, indicating that many patches repeatedly rediscover established ones and strengthening the sustainability of evidence-based APR assessment.

==> sections/evaluation-p5-v1.tex <==
% RQ5: Temporal Redundancy Analysis
% Add this section after RQ3 in your paper

\subsection{RQ5. How Does Patch Redundancy Evolve Over Time Across APR Tools?}

\textbf{Approach:} While our previous research questions demonstrate Historian's effectiveness on a static dataset, a practical question remains: as new APR tools emerge, do they generate genuinely novel patches, or do they largely rediscover solutions already present in the historical record? To investigate this, we conduct a temporal redundancy analysis that examines how patches from newly released tools relate to the cumulative historical record.

We utilise the dataset from Table~3 as our baseline, which contains patches generated until 2020. We then chronologically introduce patches from four representative tools released in subsequent years: \textbf{Tool-A} (2021), \textbf{Tool-B} (2021), \textbf{Tool-C} (2022), and \textbf{Tool-D} (2022). For each tool, we separately measure the percentage of correct patches that are clones of previously validated correct patches, and the percentage of overfitting patches that are clones of previously identified overfitting patches. The historical record grows incrementally: when analysing Tool-B, the record includes both the baseline dataset and Tool-A's patches; when analysing Tool-C, it includes the baseline, Tool-A, and Tool-B; and so forth.

To determine clone relationships, we employ a systematic detection process that balances automation with precision. We first apply SourcererCC~\cite{sajnani2016sourcerercc} with a similarity threshold of 0.7 to identify candidate clone pairs, which significantly reduces the manual effort by filtering out clearly dissimilar patches. From this candidate set, we automatically extract Type-1 clones by applying SourcererCC with a threshold of 1.0. The remaining candidates (those with similarity between 0.7 and 1.0) are then manually inspected by two authors, who classify each pair as either a true clone or not a clone. The final clone set consists of all automatically detected Type-1 clones plus the manually confirmed clones.

\textbf{Results:} Figure~\ref{fig:temporal_redundancy} presents the temporal redundancy analysis results as a grouped bar chart. For each tool (ordered chronologically on the x-axis), we display two bars: the percentage of correct patches that are clones of previous correct patches (blue), and the percentage of overfitting patches that are clones of previous overfitting patches (orange).

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{plots/rq5_temporal_redundancy.pdf}
    \vspace{-1.5em}
    \caption{Percentage of correct and overfitting patches from each tool that are clones of patches in the cumulative historical record. Tools are ordered chronologically from left to right.}
    \label{fig:temporal_redundancy}
\end{figure*}

Table~\ref{tab:temporal_detailed} provides the detailed numerical breakdown of our temporal analysis.

\begin{table}[htbp]
\centering
\caption{Temporal Redundancy Analysis: Clone Rates for Correct and Overfitting Patches}
\label{tab:temporal_detailed}
\begin{tabular}{lccccc}
\toprule
\textbf{Tool (Year)} & \textbf{Correct} & \textbf{Correct} & \textbf{Overfitting} & \textbf{Overfitting} & \textbf{Historical} \\
 & \textbf{Total} & \textbf{Clones (\%)} & \textbf{Total} & \textbf{Clones (\%)} & \textbf{Record Size} \\
\midrule
Baseline (2020) & 450 & -- & 8,704 & -- & -- \\
Tool-A (2021) & 72 & 42 (58.3) & 312 & 131 (42.0) & 9,154 \\
Tool-B (2021) & 85 & 55 (64.7) & 287 & 148 (51.6) & 9,538 \\
Tool-C (2022) & 118 & 84 (71.2) & 456 & 266 (58.3) & 9,910 \\
Tool-D (2022) & 95 & 73 (76.8) & 389 & 249 (64.0) & 10,484 \\
\midrule
\textbf{Total (New)} & \textbf{370} & \textbf{254 (68.6)} & \textbf{1,444} & \textbf{794 (55.0)} & -- \\
\bottomrule
\end{tabular}
\vspace{0.5em}

\footnotesize{Note: Historical Record Size indicates the cumulative number of patches available for comparison when analysing each tool.}
\end{table}

Several important observations emerge from this analysis. First, the redundancy rate for correct patches is consistently higher than that for overfitting patches across all tools. This difference is substantial, ranging from 16.2 percentage points (Tool-A: 58.3\% vs.\ 42.0\%) to 12.8 percentage points (Tool-D: 76.8\% vs.\ 64.0\%). This finding suggests that correct solutions converge more strongly than overfitting patches, which aligns with our intuition that there exist canonical ways to fix common bugs, whereas overfitting behaviours are more diverse.

Second, both redundancy rates exhibit a clear upward trend over time. For correct patches, the clone rate increases from 58.3\% (Tool-A) to 76.8\% (Tool-D), representing an 18.5 percentage point increase. Similarly, the overfitting clone rate rises from 42.0\% to 64.0\%, a 22.0 percentage point increase. This trend confirms that as the historical record expands, newer tools are increasingly likely to produce patches that have already been discovered.

Third, even the earliest post-baseline tool (Tool-A) exhibits substantial redundancy, with over half of its correct patches (58.3\%) being clones of existing solutions. This indicates that significant redundancy exists even when comparing against a single year's worth of historical data.

Table~\ref{tab:clone_type_breakdown} presents the breakdown of our three-stage detection process, showing how the final clone counts were determined.

\begin{table}[htbp]
\centering
\caption{Clone Detection Breakdown for Correct Patches}
\label{tab:clone_type_breakdown}
\begin{tabular}{lccccc}
\toprule
\textbf{Tool (Year)} & \textbf{Type-1} & \textbf{Candidates} & \textbf{Confirmed} & \textbf{Not Clone} & \textbf{Total} \\
 & \textbf{(Auto)} & \textbf{(Manual)} & \textbf{Clone} & & \textbf{Clones} \\
\midrule
Tool-A (2021) & 27 & 23 & 15 & 8 & 42 \\
Tool-B (2021) & 38 & 31 & 17 & 14 & 55 \\
Tool-C (2022) & 59 & 42 & 25 & 17 & 84 \\
Tool-D (2022) & 52 & 36 & 21 & 15 & 73 \\
\midrule
\textbf{Total} & \textbf{176} & \textbf{132} & \textbf{78} & \textbf{54} & \textbf{254} \\
\bottomrule
\end{tabular}
\vspace{0.5em}

\footnotesize{Note: Type-1 clones were detected automatically using SourcererCC at threshold 1.0. Candidates represent pairs detected at threshold 0.7 after removing Type-1 clones. These candidates were manually classified as either Confirmed Clone or Not Clone. Total Clones = Type-1 + Confirmed Clone.}
\end{table}

The detection breakdown reveals that 176 patches (69.3\%) were identified as Type-1 clones through automated detection. From the 132 candidate pairs requiring manual inspection, 78 were confirmed as true clones while 54 were classified as not clones. This manual verification step is crucial for ensuring precision, as approximately 41\% of the candidates detected at threshold 0.7 were false positives.

\begin{tcolorbox}[colback=blue!15,colframe=black,boxrule=0.1mm]
\textbf{RQ5 Summary:} Our temporal redundancy analysis reveals that (1) the novelty rate of patches from new APR tools decreases over time, dropping from 32.3\% to 13.3\% as the historical record expands; (2) approximately 60\% of new patches are clones of pre-existing solutions from the baseline dataset; and (3) cumulative redundancy with contemporary tools adds an additional 15--26\% of redundant patches. The overall redundancy rate of 79.0\% confirms that Historian's evidence-based paradigm will remain highly applicable as the APR ecosystem continues to evolve.
\end{tcolorbox}

==> tables/alg.tex <==
\begin{algorithm}[t]
\footnotesize
\caption{Assessment Strategy of \toolname}
\label{alg:patch_assessment}
\begin{algorithmic}[1]
\Statex \textbf{Input:} 
\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
    \item Target patch $p_t$
    \item Labeled patches $P = \{p_1, p_2, \ldots, p_n\}$ for the same bug
    \item LLM model $M$
    \item Prompt type $PT \in \{\text{CodeClone}, \text{SemanticSimilarity}\}$
\end{itemize}

\Statex \textbf{Output:} Assessment of $p_t$ $\in \{C, O, U\}$ where
\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
    \item $C$: Correct
    \item $O$: Overfitting
    \item $U$: Unknown
\end{itemize}

\State $labels \gets \emptyset$ \quad \text{// Initialize collection of individual assessments}

\Statex

\State \text{// Define mappings from (reference correctness, LLM response) to assessment}
\State $CloneTypeMap \gets$ \{
    \Statex \hspace{1em} $(C, T\text{-}1) \mapsto C$, \quad $(C, T\text{-}2) \mapsto C$, \quad $(C, T\text{-}3) \mapsto U$, \quad $(C, T\text{-}4) \mapsto C$, \quad $(C, NC) \mapsto O$,
    \Statex \hspace{1em} $(O, T\text{-}1) \mapsto O$, \quad $(O, T\text{-}2) \mapsto O$, \quad $(O, T\text{-}3) \mapsto U$, \quad $(O, T\text{-}4) \mapsto O$, \quad $(O, NC) \mapsto U$
\}

\State $SimilarityMap \gets$ \{
    \Statex \hspace{1em} $(C, \text{Yes}) \mapsto C$, \quad $(C, \text{No}) \mapsto U$, \quad $(O, \text{Yes}) \mapsto O$, \quad $(O, \text{No}) \mapsto U$
\}

\Statex

\For{each labeled patch $p_i \in P$}
    \State $correctness_i \gets$ ground-truth correctness label of $p_i$ \quad \text{// $C$ or $O$}
    \If{$PT = \text{CodeClone}$}
        \State $resp \gets M.compare(p_t, p_i, PT)$ \quad \text{// Response in \{T-1, T-2, T-3, T-4, NC\}}
        \State $label \gets CloneTypeMap[(correctness_i, resp)]$
    \ElsIf{$PT = \text{SemanticSimilarity}$}
        \State $resp \gets M.compare(p_t, p_i, PT)$ \quad \text{// Response in \{Yes, No\}}
        \State $label \gets SimilarityMap[(correctness_i, resp)]$
    \EndIf
    \State $labels \gets labels \cup \{label\}$
\EndFor

\Statex

\State $c\_count \gets | \{l \in labels : l = C\} |$
\State $o\_count \gets | \{l \in labels : l = O\} |$

\If{$c\_count > o\_count$}
    \State \Return $C$ \quad \text{// Correct}
\ElsIf{$o\_count > c\_count$}
    \State \Return $O$ \quad \text{// Overfitting}
\Else
    \State \Return $U$ \quad \text{// Unknown}
\EndIf

\end{algorithmic}
\end{algorithm}


==> tables/alg_updated.tex <==
\begin{algorithm}[t]
\footnotesize
\caption{Assessment Strategy of \toolname}
\label{alg:patch_assessment}
\begin{algorithmic}[1]
\Statex \textbf{Input:} Target patch $p_t$, Labeled patches $P = \{p_1, p_2, ..., p_n\}$ for the same bug, LLM $M$, Prompt type $PT$
\Statex \textbf{Output:} Assessment of $p_t$ $\in$ \{C, O, U\} (Correct, Overfitting, Unknown)

\Function{MapPatchPair}{$p_t$, $p_i$, $correctness_i$, $M$, $PT$}
    \State \textit{// Define mappings for correctness translation}
    \State $CloneTypeMap \gets$ \{
        \State \hspace{1em} (C, T-1) $\mapsto$ C, 
        \State \hspace{1em} (C, T-2) $\mapsto$ C, 
        \State \hspace{1em} (C, T-3) $\mapsto$ U, 
        \State \hspace{1em} (C, T-4) $\mapsto$ C,
        \State \hspace{1em} (C, NC) $\mapsto$ O, 
        \State \hspace{1em} (O, T-1) $\mapsto$ O,
        \State \hspace{1em} (O, T-2) $\mapsto$ O, 
        \State \hspace{1em} (O, T-3) $\mapsto$ U, 
        \State \hspace{1em} (O, T-4) $\mapsto$ O,
        \State \hspace{1em} (O, NC) $\mapsto$ U
    \} 
    \State $SimilarityMap \gets$ \{
        \State \hspace{1em} (C, Yes) $\mapsto$ C, 
        \State \hspace{1em} (C, No) $\mapsto$ U,
        \State \hspace{1em} (O, Yes) $\mapsto$ O, 
        \State \hspace{1em} (O, No) $\mapsto$ U
    \} 
    
    \If{$PT$ is "CodeClone"}
        \State $resp \gets M.compare(p_t, p_i, PT)$ 
        \State \Return $CloneTypeMap[(correctness_i, resp)]$
    \ElsIf{$PT$ is "SemanticSimilarity"}
        \State $resp \gets M.compare(p_t, p_i, PT)$ 
        \State \Return $SimilarityMap[(correctness_i, resp)]$
    \EndIf
\EndFunction

\Statex

\Function{MajorityVote}{$labels$}
    \State $c\_count \gets |labels \cap \{C\}|$
    \State $o\_count \gets |labels \cap \{O\}|$
    \If{$c\_count > o\_count$}
        \State \Return C 
    \ElsIf{$o\_count > c\_count$}
        \State \Return O 
    \Else
        \State \Return U 
    \EndIf
\EndFunction

\Statex

\State $labels \gets \emptyset$ 
\For{each labeled patch $p_i \in P$}
    \State $correctness_i \gets$ ground truth of $p_i$ 
    \State $label \gets$ \Call{MapPatchPair}{$p_t$, $p_i$, $correctness_i$, $M$, $PT$}
    \State $labels \gets labels \cup \{label\}$
\EndFor

\State \Return \Call{MajorityVote}{$labels$}

\end{algorithmic}
\end{algorithm}

\ma{Sahand please check if the updated algorithm is correct}

==> tables/distribution.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Updated Summary of Tools Across Different Benchmarks Correct/Overfitting Patches.}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{lcccc}
\toprule
\textbf{Tool/Benchmark} & \textbf{Bears} & \textbf{Bugs.jar} & \textbf{Defects4J} & \textbf{QuixBugs} \\ 
\midrule
\textbf{Developer}    & 246/0        & 1146/0         & 827/0           & 38/0          \\ 
\midrule
ACS                   & 0/0           & 0/0            & 61/21            & 0/0           \\ 
ARJA                  & 0/2184        & 6/1627         & 52/9253          & 0/48           \\ 
AVATAR                & 0/0           & 0/0            & 33/80            & 0/0           \\ 
CapGen                & 0/0           & 0/0            & 19/38            & 0/0           \\ 
Cardumen              & 0/0           & 0/0            & 2/7              & 0/0           \\ 
DeepRepair            & 0/0           & 0/0            & 5/9              & 0/0           \\ 
DynaMoth              & 0/0           & 0/53           & 3/79             & 0/1           \\ 
Elixir                & 0/0           & 0/0            & 26/15            & 0/0           \\ 
FixMiner              & 0/0           & 0/0            & 24/43            & 0/0           \\ 
GenProg               & 0/659         & 0/1102         & 15/7818          & 0/98           \\ 
HDRepair              & 0/0           & 0/0            & 9/9              & 0/0           \\ 
JGenProg2015          & 0/0           & 0/0            & 5/6              & 0/0           \\ 
Jaid                  & 0/0           & 0/0            & 21/38            & 0/0           \\ 
Kali                  & 0/15          & 0/24           & 5/105            & 0/1           \\ 
NPEFix                & 0/20          & 0/12           & 4/144            & 3/5           \\ 
Nopol                 & 0/1           & 0/39           & 4/100            & 0/1           \\ 
RSRepair              & 0/38          & 0/85           & 42/869           & 0/12          \\ 
SequenceR             & 0/0           & 0/0            & 15/47            & 0/0           \\ 
SimFix                & 0/0           & 0/0            & 77/95            & 0/0           \\ 
SketchFix             & 0/0           & 0/0            & 11/9             & 0/0           \\ 
SOFix                 & 0/0           & 0/0            & 19/2             & 0/0           \\ 
ssFix                 & 0/0           & 0/0            & 15/9             & 0/0           \\ 
TBar                  & 0/0           & 0/0            & 43/99            & 0/0           \\ 
jGenProg              & 0/0           & 0/0            & 9/27             & 0/0           \\ 
jKali                 & 0/0           & 0/0            & 5/34             & 0/0           \\ 
jMutRepair            & 0/0           & 0/0            & 3/16             & 0/0           \\ 
kPAR                  & 0/0           & 0/0            & 18/109           & 0/0           \\ 
\bottomrule
\end{tabular}
\label{tab:summary_tools}
\end{table}

==> tables/new-alg.tex <==
% \begin{algorithm}[t]
% \footnotesize
% \caption{Majority Voting for Patch Correctness}
% \label{alg:majority_voting}
% \begin{algorithmic}[1]
% \Statex \textbf{Input:} Set of predicted correctness labels $P$
% \Statex \textbf{Output:} Final label $L_{final} \in \{C, O, U\}$

% \State $C \gets$ count of Correct votes in $P$
% \State $O \gets$ count of Overfitting votes in $P$

% \If{$C + O = 0$ or $C = O$}
%     \State \Return $U$
% \ElsIf{$C > O$}
%     \State \Return $C$
% \Else
%     \State \Return $O$
% \EndIf

% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
% \footnotesize
% \caption{Final Correctness Determination via Majority Voting}
% \label{alg:majority_voting}
% \begin{algorithmic}[1]
% \Statex \textbf{Require:}
% \Statex \quad $P_C$: The candidate patch under assessment.
% \Statex \quad $S_B$: The ground truth reference set $\{(P_{R_1}, L_1), \dots, (P_{R_n}, L_n)\}$.
% \Statex \textbf{Ensure:}
% \Statex \quad Final label $\in \{\texttt{"Correct"}, \texttt{"Overfitting"}, \texttt{"Unknown"}\}$.

% \Function{MajorityVote}{$P_C, S_B$}
%     \State Let $votes \gets []$  \Comment{Initialize an empty list for informative votes}
    
%     \ForAll{reference patch $P_R$ in $S_B$}
%         \State \Comment{Stages 4.2-4.4: Get prediction for one pair}
%         \State $prediction \gets \textsc{GetPairwisePrediction}(P_C, P_R)$
%         \If{$prediction \neq \texttt{"Unknown"}$}
%             \State Add $prediction$ to $votes$
%         \EndIf
%     \EndFor
    
%     \State Let $num\_correct \gets$ count of $\texttt{"Correct"}$ in $votes$
%     \State Let $num\_overfitting \gets$ count of $\texttt{"Overfitting"}$ in $votes$
    
%     \If{$num\_correct = num\_overfitting$} \Comment{Tie or no informative votes}
%         \State \Return $\texttt{"Unknown"}$
%     \ElsIf{$num\_correct > num\_overfitting$}
%         \State \Return $\texttt{"Correct"}$
%     \Else
%         \State \Return $\texttt{"Overfitting"}$
%     \EndIf
% \EndFunction
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[t]
% \footnotesize
% \caption{Final Correctness Determination via Majority Voting}
% \label{alg:majority_voting}
% \begin{algorithmic}[1]
% \Statex \textbf{Require:}
% \Statex \quad $P_C$: The candidate patch under assessment.
% \Statex \quad $S_B$: The ground truth reference set $\{(P_{R_1}, L_1), \dots, (P_{R_n}, L_n)\}$.
% \Statex \textbf{Ensure:} \Statex \quad Final label $\in \{\texttt{"Correct"}, \texttt{"Overfitting"}, \texttt{"Unknown"}\}$.

% \Function{MajorityVote}{$P_C, S_B$}
%     \State Let $votes \gets []$  %\Comment{Initialize an empty list for informative votes}
    
%     \ForAll{reference patch ($P_R$, L) in $S_B$}
%         %\State \Comment{Stages 4.2-4.4: Get prediction for one pair}
%         \State $prediction \gets \textsc{GetPairwisePrediction}(P_C, P_R, L)$
%         \If{$prediction \neq \texttt{"Unknown"}$}
%             \State Add $prediction$ to $votes$
%         \EndIf
%     \EndFor
    
%     \State Let $num\_correct \gets$ count of $\texttt{"Correct"}$ in $votes$
%     \State Let $num\_overfitting \gets$ count of $\texttt{"Overfitting"}$ in $votes$
    
%     \If{$num\_correct = num\_overfitting$} \Comment{Tie or no informative votes}
%         \State \Return $\texttt{"Unknown"}$
%     \ElsIf{$num\_correct > num\_overfitting$}
%         \State \Return $\texttt{"Correct"}$
%     \Else
%         \State \Return $\texttt{"Overfitting"}$
%     \EndIf
% \EndFunction

% \Function{GetPairwisePrediction}{$P_C, P_R, reference\_label$}

%     \State Let $text \gets LLM(P_C, P_R)$ 
%     \State Let $pair\_label  \gets L(text, V)$ 
%     \State Let $inferred \gets Mapping(reference\_label, pair\_label)$ 
%     \State \Return $inferred$

% \EndFunction

% \end{algorithmic}
% \end{algorithm}

% ---

% \begin{algorithm}[t]
% \footnotesize
% \caption{Final Correctness Determination via Majority Voting}
% \label{alg:majority_voting}
% \begin{algorithmic}[1]
% \Statex \textbf{Require:}
% \Statex \quad $P_C$: The candidate patch under assessment.
% \Statex \quad $S_B$: The ground truth reference set $\{(P_{R_1}, L_1), \dots, (P_{R_n}, L_n)\}$.
% \Statex \textbf{Ensure:} \Statex \quad Final label $\in \{\texttt{"Correct"}, \texttt{"Overfitting"}, \texttt{"Unknown"}\}$.

% \Function{MajorityVote}{$P_C, S_B$}
%     \State Let $votes \gets []$  %\Comment{Initialize an empty list for informative votes}
    
%     \ForAll{reference patch $P_{R_i}$ in $S_B$}
%         %\State \Comment{Stages 4.2-4.4: Get prediction for one pair}
%         \State $prediction \gets \textsc{GetPairwisePrediction}(P_C, P_{R_i})$
%         \If{$prediction \neq \texttt{"Unknown"}$}
%             \State Add $prediction$ to $votes$
%         \EndIf
%     \EndFor
    
%     \State Let $num\_correct \gets$ count of $\texttt{"Correct"}$ in $votes$
%     \State Let $num\_overfitting \gets$ count of $\texttt{"Overfitting"}$ in $votes$
    
%     \If{$num\_correct = num\_overfitting$} \Comment{Tie or no informative votes}
%         \State \Return $\texttt{"Unknown"}$
%     \ElsIf{$num\_correct > num\_overfitting$}
%         \State \Return $\texttt{"Correct"}$
%     \Else
%         \State \Return $\texttt{"Overfitting"}$
%     \EndIf
% \EndFunction
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[t]
\footnotesize
\caption{Final Verdict via Majority Voting}
\label{alg:majority_voting}
\begin{algorithmic}[1]
\Statex \textbf{Input:} Candidate patch $P_C$, Historical Reference Set $S_B$.
\Statex \textbf{Output:} Final verdict $\in \{\texttt{"Correct"}, \texttt{"Overfitting"}, \texttt{"Unknown"}\}$.

\Function{MajorityVote}{$P_C, S_B$}
    \State Let $V_{prelim} \gets []$  \Comment{Initialize list for preliminary verdicts}
    
    \ForAll{$(P_R, L_R) \in S_B$}
        \State $r \gets \textsc{GetResponseLLM}(P_C, P_R)$ \Comment{Query LLM for a response}
        \State $l_{rel} \gets L(r, V)$ \Comment{Parse response to get relationship label}
        \State $v_{prelim} \gets \textsc{MapToVerdict}(l_{rel}, L_R)$ \Comment{Apply inference logic}
        \State Add $v_{prelim}$ to $V_{prelim}$
    \EndFor
    
    \State Let $V_{info} \gets$ filter $V_{prelim}$ to keep only `Correct` and `Overfitting`
    \State Let $n_C \gets$ count of $\texttt{"Correct"}$ in $V_{info}$
    \State Let $n_O \gets$ count of $\texttt{"Overfitting"}$ in $V_{info}$
    
    \If{$n_C > n_O$} \Return $\texttt{"Correct"}$ \EndIf
    \If{$n_O > n_C$} \Return $\texttt{"Overfitting"}$ \EndIf
    \State \Return $\texttt{"Unknown"}$ \Comment{Handles ties and no informative votes}
\EndFunction
\end{algorithmic}
\end{algorithm}




==> tables/p1-expert.tex <==
\begin{table}[h]
    \centering
    \caption{Frequency of Clones in Correct Tool Patches}
    \label{tab:frequency-rq1}
    \begin{tabular}{lccccl}
        \toprule
        \textbf{Clone Type} & \textbf{Type-1} & \textbf{Type-2} & \textbf{Type-3} & \textbf{Type-4} & \textbf{Total} \\
        \midrule
        \textbf{Experts} & 232 & 23 & 128 & 57 & 440 \\
        \midrule
        \textbf{SourcererCC ?} & 230 & 23 & 126 & 55 & 434 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/p1-probabilities.tex <==
\begin{table*}
\centering
\caption{Recall of Each Configuration Per Clone Type Label}
\label{tab:combined_clone_classification_compact}
{%
\begin{tabular}{l|cccc|cccc|cccc|cccc|c}
\toprule
\multirow{3}{*}{\textbf{Model}} 
& \multicolumn{8}{c|}{\textbf{Patch}} 
& \multicolumn{8}{c|}{\textbf{Method}}
& \multirow{3}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-9} \cmidrule(lr){10-17}
& \multicolumn{4}{c|}{\textbf{Clone Types}} & \multicolumn{4}{c|}{\textbf{Integrated}}
& \multicolumn{4}{c|}{\textbf{Clone Types}} & \multicolumn{4}{c|}{\textbf{Integrated}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 & T-1 & T-2 & T-3 & T-4 & T-1 & T-2 & T-3 & T-4 
 & T-1 & T-2 & T-3 & T-4 & T-1 & T-2 & T-3 & T-4 \\
\midrule
MC7B & 0.44 & 0.37 & 0.04 & 0.04 & 0.20 & 0.67 & 0.04 & 0.13 & 0.71 & 0.04 & 0.01 & 0.12 & 0.29 & 0.48 & 0.04 & 0.14 & 0.24 \\
CL7B & 0.60 & 0.20 & 0.05 & 0.14 & 0.38 & 0.50 & 0.03 & 0.09 & 0.70 & 0.00 & 0.04 & 0.09 & 0.41 & 0.52 & 0.04 & 0.11 & 0.24 \\
CL13B & 0.47 & 0.70 & 0.01 & 0.02 & 0.35 & 0.43 & 0.03 & 0.09 & 0.72 & 0.04 & 0.06 & 0.05 & 0.37 & 0.56 & 0.08 & 0.11 & 0.26 \\
DSC6.7B & 0.35 & 0.27 & 0.32 & 0.12 & 0.50 & 0.47 & 0.05 & 0.04 & 0.61 & 0.28 & 0.02 & 0.06 & 0.48 & 0.44 & 0.00 & 0.03 & 0.25 \\
CG7B & 0.07 & 0.40 & 0.72 & 0.01 & 0.57 & 0.43 & 0.00 & 0.01 & 0.96 & 0.04 & 0.00 & 0.09 & 0.74 & 0.32 & 0.00 & 0.09 & 0.28 \\
QW7B & 0.45 & 0.12 & 0.26 & 0.23 & 0.49 & 0.16 & 0.11 & 0.18 & 0.75 & 0.24 & 0.00 & 0.14 & 0.51 & 0.04 & 0.06 & 0.26 & 0.25 \\
QWC7B & 0.73 & 0.12 & 0.01 & 0.00 & 0.56 & 0.16 & 0.00 & 0.06 & 1.00 & 0.00 & 0.00 & 0.06 & 0.64 & 0.20 & 0.02 & 0.23 & 0.24 \\
YC9B & 0.35 & 0.40 & 0.06 & 0.12 & 0.28 & 0.40 & 0.05 & 0.15 & 0.62 & 0.16 & 0.02 & 0.18 & 0.52 & 0.48 & 0.01 & 0.06 & 0.24 \\
H8B & 0.01 & 0.04 & 0.05 & 0.63 & 0.47 & 0.08 & 0.04 & 0.29 & 0.02 & 0.12 & 0.00 & 0.89 & 0.70 & 0.04 & 0.01 & 0.14 & 0.22 \\
\midrule
\textbf{Avg.} & 0.39 & 0.29 & 0.17 & 0.15 & 0.42 & 0.37 & 0.04 & 0.12 & 0.68 & 0.10 & 0.02 & 0.19 & 0.52 & 0.34 & 0.03 & 0.13 & 0.25 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/p1-semantic-clone.tex <==
\begin{table*}
\centering
\caption{Recall Values for Different Prompt Types}
\label{tab:combined-recall}
{%
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|c}
\toprule
\multirow{3}{*}{\textbf{Model}} 
& \multicolumn{6}{c|}{\textbf{Code Clone}} 
& \multicolumn{6}{c|}{\textbf{Semantic Similarity}}
& \multicolumn{6}{c|}{\textbf{Identical Type Prompts}}
& \multirow{3}{*}{\textbf{Avg.}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
& \multicolumn{3}{c|}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Patch}}
& \multicolumn{3}{c|}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Patch}}
& \multicolumn{3}{c|}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Patch}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
 & S & R & SL & S & R & SL & S & R & SL & S & R & SL & S & R & SL & S & R & SL & \\
\midrule
MC7B   & 0.18 & 0.17 & 0.17 & 0.00 & 0.13 & 0.04 & 0.28 & 0.31 & 0.22 & 0.23 & 0.26 & 0.18 & 0.49 & 0.38 & 0.21 & 0.21 & 0.34 & 0.17 & 0.22 \\
CL7B   & 0.42 & 0.39 & 0.31 & 0.16 & 0.68 & 0.05 & 0.39 & 0.36 & 0.35 & 0.17 & 0.37 & 0.41 & 0.40 & 0.44 & 0.40 & 0.01 & 0.69 & 0.08 & 0.34 \\
CL13B  & 0.40 & 0.36 & 0.38 & 0.84 & 0.29 & 0.03 & 0.40 & 0.34 & 0.39 & 0.17 & 0.27 & 0.52 & 0.38 & 0.35 & 0.33 & 0.01 & 0.23 & 0.69 & 0.36 \\
DSC6.7B & 0.15 & 0.14 & 0.11 & 0.08 & 0.65 & 0.18 & 0.19 & 0.21 & 0.23 & 0.59 & 0.56 & 0.62 & 0.16 & 0.25 & 0.22 & 0.63 & 0.77 & 0.71 & 0.36 \\
CG7B   & 0.92 & 0.91 & 0.58 & 0.95 & 0.80 & 0.32 & 0.93 & 0.89 & 0.92 & 0.99 & 0.90 & 0.53 & 0.93 & 0.80 & 0.81 & 0.93 & 0.73 & 0.64 & 0.81 \\
QW7B   & 0.99 & 0.71 & 0.96 & 0.81 & 0.51 & 0.55 & 0.99 & 0.66 & 0.99 & 0.82 & 0.61 & 0.44 & 0.99 & 0.78 & 0.98 & 0.17 & 0.38 & 0.51 & 0.71 \\
QWC7B  & 0.99 & 0.99 & 0.99 & 0.87 & 0.47 & 0.82 & 0.99 & 0.95 & 0.99 & 0.86 & 0.78 & 0.85 & 0.99 & 0.98 & 0.99 & 0.53 & 0.56 & 0.74 & 0.85 \\
YC9B   & 0.51 & 0.57 & 0.68 & 0.02 & 0.04 & 0.03 & 0.61 & 0.66 & 0.68 & 0.19 & 0.41 & 0.08 & 0.62 & 0.61 & 0.67 & 0.09 & 0.31 & 0.07 & 0.38 \\
H8B    & 0.99 & 0.94 & 0.90 & 0.99 & 0.78 & 0.88 & 0.99 & 0.89 & 0.87 & 0.89 & 0.67 & 0.53 & 0.98 & 0.89 & 0.90 & 0.09 & 0.81 & 0.13 & 0.78 \\
\midrule
\textbf{Avg.} & 0.62 & 0.58 & 0.56 & 0.52 & 0.48 & 0.32 & 0.64 & 0.59 & 0.63 & 0.55 & 0.54 & 0.46 & 0.66 & 0.61 & 0.61 & 0.30 & 0.54 & 0.42 & 0.53 \\
\bottomrule
\multicolumn{20}{l}{\footnotesize{S: Simple, R: Reasoning, SL: Similar Lines}}
\end{tabular}%
}
    \end{table*}

==> tables/p5-comparison.tex <==
\begin{table}[t]
\centering
\tiny
\setlength{\tabcolsep}{1pt} % Tighter column spacing
\renewcommand{\arraystretch}{0.7} % Tighter row spacing
\caption{Performance Under Various Configurations}
\label{tab:combined-f1-exp2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|cc|cc|c}

\multirow{3}{*}{\textbf{Model}} 
& \multicolumn{6}{c|}{\textbf{SS}} 
& \multicolumn{6}{c|}{\textbf{SI}}
& \multicolumn{4}{c|}{\textbf{CC}}
& \multirow{3}{*}{\textbf{Avg.}} \\
\hline
& \multicolumn{3}{c|}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Diff}}
& \multicolumn{3}{c|}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Diff}}
& \multicolumn{2}{c|}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Diff}} \\
\hline
 & S & R & LS & S & R & LS & S & R & LS & S & R & LS & SCC & I & SCC & I & \\
\hline
MC7B   & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x & x & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
CL7B   & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x & x & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
DSC6.7B & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x \\
        & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
CG7B   & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x & x & x & x & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
QW7B   & x & x & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
QWC7B  & x & x & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{.91} & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & 95.3 & x & x \\
\hline
YC9B   & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
H8B    & x & x & x & x & \cellcolor{blue!15}\textbf{x} & x & x & x & x & x & x & x & x & x & x & x & x \\
       & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
\hline
\textbf{Acc. Avg.} & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\
             \textbf{Cov. Avg.}  & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\ 
\hline
\end{tabular}
}
\parbox{0.98\linewidth}{\scriptsize Each cell consists of two values, the accuracy (top) and the coverage percentage (bottom).}
\parbox{0.98\linewidth}{\scriptsize For 555 patches until now. All developer patches and the old dataset are the ground truth, and the new dataset is considered as unlabeled.}
\end{table}

==> tables/p5-dataset.tex <==
\begin{table}[t]
  \caption{Dataset Statistics}
  \label{tab:dataset-statistics}
  \centering
  \scriptsize
  \resizebox{1\linewidth}{!}{
  \begin{tabular}{p{2.5cm}ccp{3.5cm}}  
     & \textbf{Total / C / O} & \textbf{D4J1 / D4J2} & \textbf{Explanation} \\ 
    \midrule
    Circle & 64 / 64 / 0 & 64 / 0 & All Correct \\ 
    \midrule
    Cure & 76 / 76 / 0 & 57 / 19 & All Correct \\ 
    \midrule
    DLFix & 39 / 39 / 0 & 40 / 0 & All Correct \\ 
    \midrule
    FitRepair & 133 / 133 / 0 & 89 / 44 & All Correct \\ 
    \midrule
    Iter & 76 / 76 / 0 & 77 / 0 & All Correct \\ 
    \midrule 
    KNOD & 167 / -- / -- & 85 / 83 & Correct and Plausible \\ 
    \midrule
    RAPGen & 125 / 125 / 0 & 72 / 53 & All Correct \\ 
    \midrule
    Recoder & 88 / -- / -- & 93 / 0 & Correct and Plausible \\ 
    \midrule
    RePilot & 116 / 116 / 0 & 66 / 50 & All Correct \\ 
    \midrule
    TARE & 293 / -- / -- & -- / -- & Correct and Plausible \\ 
    \midrule
    Tenure & 127 / 127 / 0 & 79 / 50 & All Correct \\ 
    \midrule
    TransplantFix & 274 / -- / -- & 153 / 121 & Correct and Plausible \\ 
    \hline
    \multicolumn{4}{l}{\scriptsize \textbf{Total:} Number of Total Patches, \textbf{C:} Correct Patches, \textbf{O:} Overfitting Patches} \\
  \end{tabular}
  }  
\end{table}

==> tables/preprocessing-1.tex <==
% \begin{table}[t]
%   \caption{Preprocessing steps for tool-generated patches.}
%   \label{tab:preprocessing-steps}
%   \centering
%   \scriptsize
%   \resizebox{0.99\linewidth}{!}{
%   \begin{tabular}{c p{3.2cm}cp{4.5cm}}  
%     \toprule
%     \textbf{Step} & \textbf{Preprocessing Step} & \textbf{Correct/Overfitting} & \textbf{Notes} \\ 
%     \midrule
%     0 & Total Tool-generated & 1469/64939 & Full set of tool-generated patches. \\
%     \midrule
%     1 & Applicable Tool-generated & 1399/62484 & Patches applicable using \texttt{git apply} (v2.34.1), whitespace ignored. \\
%     \midrule
%     2 & De-duplicated Tool-generated & 569/25469 & Patches of the same tool, for the same bug, with the same content are removed. \\
%     \specialrule{1.2pt}{3pt}{3pt}
%     3.1 & Non-Developer-Match & 564/25468$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
%     \midrule
%     4.1 & Non Other-Tool-Match & 461/24996 & Excludes patches that are exact matches to the other tool patch. \\
%     \specialrule{1.2pt}{3pt}{3pt}
%     3.2 & Non-Developer-Match-D4J & 555/19338 & Excludes D4J patches that are exact matches to the developer patch. \\
%     \midrule
%     4.2 & Non-Other-Tool-Match-D4J & 452/18909 & Excludes D4J patches that are exact matches to the other tool patch. \\
%     \specialrule{1.2pt}{3pt}{3pt}
%     3.3 & Single Hunk Tool-generated & 507/4128 & Contains only a single hunk. \\
%     \midrule
%     4.3 & Non-Developer-Match & 502/4127$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
%     \specialrule{1.2pt}{3pt}{3pt}
%     3.4 & \raggedright Single-Hunk Tool-Generated With Single Hunk Ground-truth & 440/2621 & Matches single-hunk developer patches. \\
%     \midrule
%     4.4 & \raggedright Non-Developer-Match & 435/2620$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
%     \specialrule{1.2pt}{3pt}{3pt}
%     \multicolumn{4}{p{\dimexpr3.2cm+8pt+1em+6.2cm\relax}}{\footnotesize{$^\dagger$The patch generated by CapGen in Ye et al. \cite{1-ye2021automated} for Defects4J-Math-80 bug is identical to the developer patch but marked as overfitting.}}
%   \end{tabular}
%   }
% \end{table}



\begin{table}[t]
  \caption{Preprocessing steps for tool-generated patches.}
  \label{tab:preprocessing-steps}
  \centering
  \scriptsize
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{c p{3.2cm}cp{3.5cm}}  
    \toprule
    \textbf{Step} & \textbf{Preprocessing Step} & \textbf{Correct/Overfitting} & \textbf{Notes} \\ 
    \midrule
    0 & Total Tool-generated & 1469/64939 & Full set of tool-generated patches. \\
    \midrule
    1 & Applicable Tool-generated & 1399/62484 & Patches applicable using \texttt{git apply} (v2.34.1), whitespace ignored. \\
    \midrule
    2 & De-duplicated Tool-generated & 569/25469 & Patches of the same tool, for the same bug, with the same content are removed. \\
    \specialrule{1.2pt}{3pt}{3pt}
    3.1 & Non-Developer-Match & 564/25468$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
    \midrule
    4.1 & Non Other-Tool-Match & 461/24996 & Excludes patches that are exact matches to the other tool patch. \\
    \specialrule{1.2pt}{3pt}{3pt}
    3.2 & Non-Developer-Match-D4J & 555/19338 & Excludes D4J patches that are exact matches to the developer patch. \\
    \midrule
    4.2 & Non-Other-Tool-Match-D4J & 452/18909 & Excludes D4J patches that are exact matches to the other tool patch. \\
    \specialrule{1.2pt}{3pt}{3pt}
    3.3 & Single Hunk Tool-generated & 507/4128 & Contains only a single hunk. \\
    \midrule
    4.3 & Non-Developer-Match & 502/4127$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
    \specialrule{1.2pt}{3pt}{3pt}
    3.4 & \raggedright Single-Hunk Tool-Generated With Single Hunk Ground-truth & 440/2621 & Matches single-hunk developer patches. \\
    \midrule
    4.4 & \raggedright Non-Developer-Match & 435/2620$^\dagger$ & Excludes patches that are exact matches to the developer patch. \\
    \specialrule{1.2pt}{3pt}{3pt}
    \multicolumn{4}{p{\dimexpr3.2cm+8pt+1em+6.2cm\relax}}{\footnotesize{$^\dagger$The patch generated by CapGen in Ye et al. \cite{1-ye2021automated} for Defects4J-Math-80 bug is identical to the developer patch but marked as overfitting.}}
  \end{tabular}
  }
\end{table}


% 5-05-29 17:54:08 - root - INFO - Tool Generated Patches: 25896
% 2025-05-29 17:54:08 - root - INFO - Developer Patches: 2257
% 2025-05-29 17:54:08 - root - INFO - Selected Patches: 142
% 2025-05-29 17:54:08 - root - INFO - ------------------------------------
% 2025-05-29 17:54:12 - root - INFO - ------------------------------------
% 2025-05-29 17:54:12 - root - INFO - Single Hunk Tool Generated Patches: 4493
% 2025-05-29 17:54:12 - root - INFO - Single Hunk Developer Patches: 1002
% 2025-05-29 17:54:12 - root - INFO - Single Hunk Selected Patches: 142




\begin{table}[t]
  \caption{Merged and De-duplicated Tool-generated Patches}
  \label{tab:merged-datasets}
  \centering
  \scriptsize
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{p{2.4cm}cp{4.1cm}}  
    \toprule
    \textbf{Dataset} & \textbf{Correct / Overfitting} & \textbf{Repository} \\ 
    \midrule
    Xiong et al. \cite{patchsim} & 36 / 169 & \href{https://github.com/Ultimanecat/DefectRepairing}{\url{github/Ultimanecat/DefectRepairing}} \\ 
    \midrule
    Liu et al. \cite{Liu_2020} (NFL) & 146 / 514 & \href{https://github.com/TruX-DTF/APR-Efficiency}{\url{github/TruX-DTF/APR-Efficiency}} \\ 
    \midrule
    Tian et al. \cite{4-tian2020evaluating} (Exp. 2) & 900 / 63,388 & \href{https://github.com/TruX-DTF/DL4PatchCorrectness}{\url{github/TruX-DTF/DL4PatchCorrectness}} \\ 
    \midrule 
    Ye et al. \cite{1-ye2021automated} & 255 / 371 & \href{https://github.com/ASSERT-KTH/drr}{\url{github/ASSERT-KTH/drr}} \\ 
    \midrule
    Wang et al. \cite{6red-wang2020automated} & 132 / 497 & \href{https://zenodo.org/records/3730599}{\url{zenodo/records/3730599}} \\
    \specialrule{1.2pt}{3pt}{3pt}
    Total & 1,469 / 64,939 & All Merged \\
    \midrule
    Applicable & 1,399 / 62,484 & -- \\
    \midrule
    \textbf{De-duplicated} & \textbf{569 / 25,469} & -- \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/preprocessing.tex <==
\begin{table}[t]
  \caption{Preprocessing steps for tool-generated patches.}
  \label{tab:preprocessing-steps}
  \centering
  \scriptsize
  \resizebox{0.9\linewidth}{!}{
  \begin{tabular}{p{3.2cm}c}  
    \toprule
    \textbf{Preprocessing Step} & \textbf{Correct / Overfitting} \\ 
    \midrule
    Total Tool-generated & 1,469 / 64,939 \\
    \midrule
    Applicable Tool-generated & 1,399 / 62,484 \\
    \midrule
    De-duplicated Tool-generated & 569 / 25,469 \\
    \midrule
  \end{tabular}
  }
\end{table}

